Development and Implementation of Advanced Beam Diagnostic and Abort Systems in SuperKEKB

The SuperKEKB/Belle II experiment aims to collect high-statistics data of B meson pairs to explore new physics beyond the Standard Model (SM). SuperKEKB, an upgraded version of the KEKB accelerator, has achieved a world-record luminosity of $4.71 \times 10^{34} \, \mathrm{cm^{-2}s^{-1}}$ in 2022 but continues to strive for higher luminosities. One of the major obstacles is Sudden Beam Loss (SBL) events, which cause substantial beam losses and damage to the Belle~II detector. To find a hint for addressing SBL challenges, advanced beam diagnostic systems and enhanced beam abort systems have been developed. The diagnostic system aims to accurately pinpoint the start of beam losses, while the upgraded abort system quickly disposes of anomalous beams to minimize damage. This paper details the development and implementation of these systems, including high-speed loss monitors, time synchronization with the White Rabbit system, and data acquisition systems. Efforts to understand the mechanisms of SBL events, using acoustic sensors to detect discharges, are also discussed. These measures aim to improve the operational stability and luminosity of SuperKEKB, contributing to the experiment's success.

==> sections/claws_install.tex <==
We installed four CLAWS sensors around the newly constructed vertical collimator in the D05 area. 
Figure \ref{fig:CLAWSatD05V1} is a picture of the beamline around the collimator.
One sensor was installed upstream from the collimator while the remaining three were installed downstream.

In the operation of February and March 2024, we carried out the commissioning of new CLAWS sensors.
Figure \ref{fig:d05claws_signal} shows a typical signal in the case of the beam loss abort.
In general, the sensors \#1 (upstream) and \#4 (most downstream) observe relatively larger beam loss as shown in this picture.
On the other hand, in the case of the SBL accidents, the beam loss around this collimator becomes huge. Therefore, the signal from all CLAWS sensors are saturated.

We selected the sensor \# 2 for the abort sensor.
It is to ensure the wide threshold range for the abort request condition.
As a reality, the abort request threshold has been optimized with increase of the operation beam current.
The threshold was implemented to be 35\,mV at first.
However, it was increased up to 100\,mV in the end of 2024 spring run period.

In addition to the threshold, we implemented the signal duration to the abort request condition. It is effective condition that we select SBLs from any other beam loss or noise. It is well known that the huge beam loss continues more than 1 $\mu$s in the case of SBL.
The abort request signal is launched when the beam loss waveform exceeds longer than xxx ns.

We implemented the injection veto to the abort request logic of the CLAWS at D05. 
The launch of the abort request signal has been vetoed during 1\,ms from the injection.
This conidition was optimized during the 2024 spring operation.


%In the betatron injection scheme at SuperKEKB, the injected bunch is merged with the storage bunch with the radiation damping.

%During this period, the injection bunch irradiates, and the short-distance beam loss is observed periodically.

%We understand it continued for longer than 10\,ms.

From March 23 to March 27 in 2024, We carried out the feasibility test with the above abort request condition.

We provided the pseudo-abort request with the new CLAWS abort sensor. 

Its response time was compared with that of the abort trigger system in operation. 

Table \ref{tab:claws_feas} shows the list of the positron beam aborts which the CLAWS launched the pseudo-abort request at the same time.

The time interval of two signal is measured in two levels.
One is the comparison of the arrival timing of the two request signal at CCB. The other is the arrival timing of the abort kicker trigger at the power supply station at D07.
Most of aborts, the pseudo-abort request is faster than that in operation.
The time difference depends on which sensor firstly launched the abort request.
In the best case, the abort kicker trigger generated from CLAWS at D05 is 45 $\mu$ faster. It corresponds to 4 turn and half.
Therefore, the test result obviously evaluated the feasibility of new CLAWS sensor.

Only once, the pseudo-abort request has been launched alone during this test period.
This event can be doubted as an unnecessary abort request that disturbs the SuperKEKB beam operation.
However, its frequency, once in a week, is acceptable in terms of our beam operation and commissioning.

After confirming the feasibility of the new CLAWS sensor, we integrated it as the abort sensor at the SuperKEKB positron ring on March 27 2024.



\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/CLAWSatD05V1.png}
    \caption{D05 vertical collimator and CLAWS sensor: the vertical collimator is highlighted with the large red circle. It is called Non Linear Collimator. The position of the CLAWS sensor is highlighted with the small circle.}
    \label{fig:CLAWSatD05V1}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/d05claws_signal.png}
    \caption{An example of signals from CLAWS at D05V1:}
    \label{fig:d05claws_signal}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{ccccc}
Date \& Time & 1st source & \multicolumn{2}{c}{$\Delta$ t ($\mu$s)}& Mitigation \\
& & D07 & CCB & \\
\hline
03-23 07:08 &CLAWS &-10 &-8 &No\\
03-23 09:14 &D06V1Pin &-10 &-8 &No\\
03-23 13:48 &CLAWS &-25 &-21 &No\\
03-23 15:40 &CLAWS &-5 &-3 &Yes\\
03-23 17:17 &CLAWS &-10 &-8 &Yes\\
03-23 18:26 &Fiber &+5 &+5 &No\\
03-24 08:03 &CLAWS &-5 &-3 &No\\
03-24 16:58 &D06V1Pin &-5 &0 &No\\
03-24 20:47 &D06V1Pin &-15 &-15 &No\\
03-24 21:04 &CLAWS &-5 &-7 &Yes\\
03-25 07:47 &CLAWS &-15 &-15 &Yes\\
03-25 14:07 &CLAWS &-5 &-4 &Yes\\
03-25 16:23 &CLAWS &-5 &-6 &No\\
03-25 18:05 &CLAWS &-10 &-10 &No\\
03-25 18:41 &D06V1Pin &-15 &-14 &No\\
03-27 04:11 &Fiber &-45 &-46 &No\\
03-27 06:12 &D06V1Pin &-35 &-36 &No\\
03-28 05:26 &Fiber &-25 &-23 &Yes\\      
    \end{tabular}
    \caption{Time interval between abort request in operation and psuedo-abort request launched by new CLAWS: Note, that abort kicker trigger is synchronized with the bunch train gap that comes every 5\,$\mu$s. Therefore, the time interval of the abort kicker trigger becomes a multiple of 5\,$\mu$s.}
    \label{tab:claws_feas}
\end{table}

